Neural Networks with Sparse Activation Induced by Large Bias: Tighter Analysis with Bias-Generalized NTK

We study training one-hidden-layer ReLU networks in the neural tangent kernel (NTK) regime, where the networks' biases are initialized to some constant rather than zero. We prove that under such initialization, the neural network will have sparse activation throughout the entire training process, which enables fast training procedures via some sophisticated computational methods. With such initialization, we show that the neural networks possess a different limiting kernel which we call \textit{bias-generalized NTK}, and we study various properties of the neural networks with this new kernel. We first characterize the gradient descent dynamics. In particular, we show that the network in this case can achieve as fast convergence as the dense network, as opposed to the previous work suggesting that the sparse networks converge slower. In addition, our result improves the previous required width to ensure convergence. Secondly, we study the networks' generalization: we show a width-sparsity dependence, which yields a sparsity-dependent Rademacher complexity and generalization bound. To our knowledge, this is the first sparsity-dependent generalization result via Rademacher complexity. Lastly, we study the smallest eigenvalue of this new kernel. We identify a data-dependent region where we can derive a much sharper lower bound on the NTK's smallest eigenvalue than the worst-case bound previously known. This can lead to improvement in the generalization bound.

==> discussion.tex <==
\section{Discussion}
In this work, we study training one-hidden-layer overparameterized ReLU networks in the NTK regime where its biases initialized as some constants rather than zero so that its activation remains sparse during the entire training process. 
We showed an improved sparsity-dependent results on convergence, generalization and restricted least eigenvalue. 
One immediate future direction is to generalize our analysis to multi-layer neural networks. 
On the other hand, in practice, label shifting is never used. 
Although we show that the least eigenvalue can be much better than previous result when we impose additional assumption of the restricted region, an open problem is whether it is possible to improve the infinite-width NTK's least eigenvalue's dependence on the sample size without such assumption, or even whether a lower bound purely dependent on the data separation is possible so that the worst-case generalization bound doesn't scale with the sample size. 
We leave these questions as future work. 
